Bayesian Error-in-Variables Models for the Identification of Power Networks

The increasing integration of intermittent renewable generation, especially at the distribution level,necessitates advanced planning and optimisation methodologies contingent on the knowledge of thegrid, specifically the admittance matrix capturing the topology and line parameters of an electricnetwork. However, a reliable estimate of the admittance matrix may either be missing or quicklybecome obsolete for temporally varying grids. In this work, we propose a data-driven identificationmethod utilising voltage and current measurements collected from micro-PMUs. More precisely,we first present a maximum likelihood approach and then move towards a Bayesian framework,leveraging the principles of maximum a posteriori estimation. In contrast with most existing con-tributions, our approach not only factors in measurement noise on both voltage and current data,but is also capable of exploiting available a priori information such as sparsity patterns and knownline parameters. Simulations conducted on benchmark cases demonstrate that, compared to otheralgorithms, our method can achieve significantly greater accuracy.

==> OLS_TLS.tex <==
\begin{figure}[H]
    \centering
    \hspace{0.1cm}
    \begin{subfigure}[t]{0.12\textwidth}
        \begin{tikzpicture}[scale=0.7]
        \begin{axis}[
            axis lines=middle,
            axis equal image,
            xtick=\empty, ytick=\empty,
            enlargelimits=true,
            clip mode=individual, clip=false
            ]
            \addplot [RoyalBlue, mark=none, thick, opacity=0] coordinates {(-0.1, -1) (0.1, 1)};
            \addplot [ForestGreen, mark=none, thick] coordinates {(-0.5, 0.2) (0.5, -0.2)};
            
            \addplot [black, only marks, mark=*, mark size=1.5] coordinates {(-0.1, -0.6) (0.1, 0.6)};
            \addplot [black, only marks, mark=*, mark size=20, opacity=0.2] coordinates {(-0.1, -0.6) (0.1, 0.6)};
            
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(-0.1, -0.5) (-0.1, 0.04)};
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(-0.15, 0.7) (-0.15, 0.06)};
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(0.0, -0.6) (0.0, 0.0)};
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(0.15, 0.5) (0.15, -0.06)};
            
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(-0.1, -0.5) (-0.15, 0.7)};
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(0.0, -0.6) (0.15, 0.5)};
        \end{axis}
        \end{tikzpicture}
        \caption{OLS regression with high slope and EIV}
        \label{fig:graph_ols}
    \end{subfigure}
    \begin{subfigure}[t]{0.12\textwidth}
        \begin{tikzpicture}[scale=0.7]
        \begin{axis}[
            axis lines=middle,
            axis equal image,
            xtick=\empty, ytick=\empty,
            enlargelimits=true,
            clip mode=individual, clip=false
            ]
            \addplot [RoyalBlue, mark=none, thick] coordinates {(-0.1, -1) (0.1, 1)};
            \addplot [ForestGreen, mark=none, thick, opacity=0] coordinates {(-0.5, 0.2) (0.5, -0.2)};
            
            \addplot [black, only marks, mark=*, mark size=1.5] coordinates {(-0.1, -0.6) (0.1, 0.6)};
            \addplot [black, only marks, mark=*, mark size=20, opacity=0.2] coordinates {(-0.1, -0.6) (0.1, 0.6)};
            
            \addplot [RoyalBlue, mark=none, opacity=0.8] coordinates {(-0.1, -0.5) (-0.05, -0.505)};
            \addplot [RoyalBlue, mark=none, opacity=0.8] coordinates {(-0.15, 0.7) (0.06, 0.68)};
            \addplot [RoyalBlue, mark=none, opacity=0.8] coordinates {(0.0, -0.6) (-0.06, -0.595)};
            \addplot [RoyalBlue, mark=none, opacity=0.8] coordinates {(0.15, 0.5) (0.05, 0.51)};
            
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(-0.1, -0.5) (-0.15, 0.7)};
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(0.0, -0.6) (0.15, 0.5)};
        \end{axis}
        \end{tikzpicture}
        \caption{TLS regression with high slope and EIV}
        \label{fig:graph_tls}
    \end{subfigure}
    \begin{subfigure}[t]{0.2\textwidth}
        \begin{tikzpicture}[scale=0.7]
        \begin{axis}[
            axis lines=middle,
            axis equal image,
            xtick=\empty, ytick=\empty,
            enlargelimits=true,
            clip mode=individual, clip=false
            ]
            \addplot [black, only marks, mark=*, mark size=1.5] coordinates {(0.0, 0.0)};
            \addplot [black, only marks, mark=*, mark size=60, opacity=0.2] coordinates {(0.0, 0.0)};
            
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(-0.7, -0.7) (-0.7, 0.7)};
            \addplot [ForestGreen, mark=none, opacity=0.8] coordinates {(0.7, -0.7) (0.7, 0.7)};
            \addplot [RoyalBlue, mark=none, opacity=0.8] coordinates {(-0.7, 0.7) (0.7, -0.7)};
            
            \addplot [RoyalBlue, mark=none, thick] coordinates {(-1.2, -1.2) (1.2, 1.2)};
            \addplot [ForestGreen, mark=none, thick] coordinates {(-1.2, 0) (1.2, 0)};
            
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(-0.7, -0.7) (-0.7, 0.7)};
            \addplot [red, only marks, mark=*, mark size=1.5] coordinates {(0.7, -0.7) (0.7, 0.7)};
        \end{axis}
        \end{tikzpicture}
        \caption{OLS and TLS for uncorrelated data with EIV}
        \label{fig:graph_tls_ols_uncorr}
    \end{subfigure}
    \caption{Worst and best cases for two estimation methods.}
    \label{fig:ols_tls_comp_graph}
\end{figure}

==> comparison.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}[scale=0.8]

\definecolor{color0}{rgb}{0.00392156862745098,0.0023529411764706,0.003137254901961}
\definecolor{color1}{rgb}{0.204901960784314,0.311764705882353,0.802352941176471}
\definecolor{color2}{rgb}{0.133333333333333,0.545098039215686,0.133333333333333}
\definecolor{color3}{rgb}{0.803921568627451,0.52156862745098,0.247058823529412}

\begin{axis}[
legend cell align={left},
legend columns=2,
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(1,0.22)}, anchor=east, draw=white!80!black},
tick align=outside,
tick pos=left,
width=\textwidth,
height=0.4\textwidth,
xmajorgrids,
xmin=-2.7, xmax=56.7,
xminorgrids,
minor tick num=4,
xtick style={color=black},
ymin=-807.528819634138, ymax=17342.860399576,
ytick style={color=black}
]
\addplot [line width=1pt, red!54.5098039215686!black, mark=*, mark size=4, mark options={solid}]
table {%
0 7553.84480715581
1 5665.38352269083
2 11330.7672160249
3 7553.84480715581
4 5665.38352269083
5 2746.8526036227
6 11330.7672160249
7 4548.55166804551
8 3573.86203074499
9 8240.55775069638
10 1624.48267785601
11 3021.53791129209
12 5629.9905529994
13 6474.72395757788
14 8042.84368247639
15 4021.42184123819
16 3311.75915481413
17 4330.76200482522
18 8240.55775069638
19 2832.69174001501
20 3115.96096052673
21 11330.7672160249
22 5665.38352269083
23 3237.36203321338
24 6085.78288155211
25 2882.7392707355
26 1281.21750391789
27 4770.84927883616
28 9064.61366106848
29 9064.61366106848
30 5035.89650596432
31 8240.55775069638
32 10071.7928833705
33 10071.7928833705
34 7553.84480715581
35 4120.27892047698
36 2832.69174001501
37 7553.84480715581
38 8240.55775069638
39 6972.77972756124
40 7553.84480715581
41 6043.07582258417
42 9064.61366106848
43 8240.55775069638
44 11330.7672160249
45 7553.84480715581
46 6474.72395757788
47 9064.61366106848
48 9064.61366106848
49 11330.7672160249
50 9064.61366106848
51 15107.6893250557
52 9064.61366106848
53 9064.61366106848
54 9064.61366106848
};
\addlegendentry{exact}
\addplot [only marks, color0, mark=square*, mark size=4, mark options={solid}]
table {%
0 227.033461596583
1 614.647245559694
2 274.199227231602
3 238.589897016349
4 154.097084499388
5 62.7886746715934
6 170.958281410689
7 61.1233927560474
8 98.9969988827664
9 189.890233113958
10 38.8722863645134
11 62.0001859924242
12 107.344952774948
13 183.956250052332
14 229.87566461839
15 119.701095953306
16 98.486631877124
17 130.530263157937
18 184.318294719119
19 49.9839473949955
20 90.3713096882465
21 358.705078410041
22 218.401611679676
23 201.390928983159
24 160.899154504207
25 51.8259988711216
26 21.48128465644
27 38.2729167261913
28 92.0315892717074
29 124.216776235316
30 178.726320615336
31 177.567000146301
32 68.0808944563817
33 62.8094548970961
34 131.844598138389
35 86.1490334283153
36 51.8782788180308
37 198.264383593137
38 170.694312097587
39 94.3475591773738
40 206.415131665729
41 138.839983086997
42 140.720507318907
43 125.312869966189
44 144.624261335657
45 75.2496103348365
46 130.991762471506
47 290.839706521535
48 137.389713000806
49 178.140869335606
50 62.9670764376714
51 256.471973918636
52 70.5958377811598
53 155.221240908172
54 211.407146391039
};
\addlegendentry{OLS}
\addplot [only marks, color1, mark=halfsquare*, mark size=4, mark options={solid}]
table {%
0 5614.50084317375
1 5370.42114766296
2 11732.0178126527
3 8647.3755633505
4 5796.34108150028
5 2607.05117232916
6 11901.642933888
7 4700.4434101489
8 3984.30972879746
9 7077.67127332955
10 639.240353264926
11 2418.45946136685
12 6031.02245223883
13 7422.86915543656
14 9026.6770631466
15 3874.7163736571
16 3185.39445380912
17 4367.56941442073
18 7418.39649453875
19 2517.09016801553
20 3860.44728409833
21 11396.8183859487
22 5423.71869524153
23 3871.9483574596
24 5729.71542829287
25 3684.84764637685
26 603.046548734424
27 4472.49528694813
28 8965.08270474328
29 8362.44563387272
30 5477.88568700946
31 9418.62996423986
32 8948.38511981169
33 10190.2996710592
34 7259.78453545154
35 4055.20569989203
36 2281.96418489782
37 7567.31073388869
38 8690.57513122727
39 7488.33049630105
40 6824.01407453799
41 6229.80087735962
42 6649.4573250571
43 7850.70478770464
44 11877.2232176337
45 8231.25512626454
46 6525.26341361963
47 8076.07975650261
48 7699.48981768018
49 8985.72149215256
50 8928.1294027088
51 15650.1758977289
52 8523.18850121163
53 8026.26144322109
54 9162.46720717914
};
\addlegendentry{TLS}
\addplot [only marks, color2, mark=triangle*, mark size=4, mark options={solid}]
table {%
0 181.485625703514
1 736.181929985028
2 226.245403658608
3 261.140819123399
4 156.35379360729
5 73.4863523299545
6 159.158240874691
7 45.4367902893441
8 99.4369907360431
9 153.453055159223
10 32.2425078537976
11 57.194327793693
12 91.0379447373305
13 179.90435026154
14 213.562475367174
15 129.030366078855
16 166.320306613321
17 170.986545081366
18 154.497323468535
19 48.2393739282146
20 105.30398014523
21 467.849854113651
22 300.507965959444
23 260.80757969726
24 112.33580436105
25 43.974077904729
26 17.4888721481421
27 48.7949492592082
28 114.323231983863
29 95.3398729564998
30 169.311711422481
31 190.674341626302
32 58.9105576806538
33 56.9239510184437
34 124.213992223743
35 91.6277066267423
36 46.5048754430877
37 183.676528490429
38 153.84390048164
39 88.1331342326697
40 191.701643480268
41 165.503031170887
42 123.547258718581
43 129.37027847421
44 148.918132916867
45 66.963665201793
46 121.686764558645
47 276.077229514549
48 121.79029111205
49 198.061941477631
50 22.6090001748316
51 338.335409165067
52 49.5421884313114
53 165.767563433623
54 165.921523393278
};
\addlegendentry[align=left]{adaptive Lasso}
\addplot [only marks, color3, mark=diamond*, mark size=4, mark options={solid}]
table {%
0 6415.07486652436
1 5616.28300942736
2 11511.8996157483
3 8340.05459999902
4 5827.89325480923
5 2480.5304748739
6 11250.971190022
7 5232.56025125019
8 4287.05293512638
9 6927.15717945625
10 34.8603653597199
11 3097.31942809846
12 6167.81786301151
13 6602.2078716671
14 8668.10369136628
15 3901.64109217149
16 3187.93891463734
17 4381.77055923133
18 8381.91897003219
19 2958.49852507154
20 2578.25269511592
21 11039.814966467
22 6186.26319124784
23 3393.42877206427
24 5524.93763160008
25 2886.15611684147
26 1455.79503551246
27 4550.63428254607
28 8986.72462743558
29 8306.46173544018
30 5214.83797157635
31 8658.27779391198
32 8822.40517304187
33 9985.03615530783
34 7069.29711562771
35 4255.2743909222
36 2375.40479908968
37 7435.51921931587
38 8842.88587749055
39 7238.20165296448
40 7242.24652732092
41 6381.80452852269
42 6790.51663883423
43 8292.01322381171
44 11520.6849296299
45 7681.80134191694
46 6459.97818598234
47 7858.75543184479
48 8405.79594549172
49 10058.8085376502
50 7694.68656020961
51 16517.8427077937
52 9133.28155989982
53 8910.59028987168
54 9061.28928951397
};
\addlegendentry{MAP}
\end{axis}

\end{tikzpicture}


